Dimension of polynomial splines of mixed smoothness on T-meshes

In this paper we study the dimension of splines of mixed smoothness on axis-aligned T-meshes. This is the setting when different orders of smoothness are required across the edges of the mesh. Given a spline space whose dimension is independent of its T-mesh's geometric embedding, we present constructive and sufficient conditions that ensure that the smoothness across a subset of the mesh edges can be reduced while maintaining stability of the dimension. The conditions have a simple geometric interpretation. Examples are presented to show the applicability of the results on both hierarchical and non-hierarchical T-meshes. For hierarchal T-meshes it is shown that mixed smoothness spline spaces that contain the space of PHT-splines (Deng et al., 2008) always have stable dimension.

==> setup/commands_simp.tex <==
%%%%%% NEW COMMANDS %%%%%%%%


\newcommand{\degreeDiff}{d^\face}

\newcommand{\minDegreeu}{{\check{\degreeu}}}
\newcommand{\minDegreev}{{\check{\degreev}}}
\newcommand{\maxDegreeu}{{\bar{\degreeu}}}
\newcommand{\maxDegreev}{{\bar{\degreev}}}
\newcommand{\polyTotal}[1]{\mathbb{P}_{#1}}
\newcommand{\polyRing}{R}
\newcommand{\polyRingH}{S}
\newcommand{\ideal}{\mathfrak{J}}
\newcommand{\idealL}{\mathfrak{L}}
\newcommand{\shiftideal}[3]{\mathfrak{#1}_{#2}(#3)}


\newcommand{\krond}[2]{\varepsilon_{#1, #2}}
\newcommand{\kronFE}[2]{\krond{\face_{#1}}{\edge_{#2}}}
\newcommand{\kronEV}[2]{\krond{\edge_{#1}}{\vertex_{#2}}}


==> setup/commands_tmesh.tex <==

%%%%%% NEW COMMANDS %%%%%%%%

%% T-mesh
\newcommand{\ids}{\chi}
\newcommand{\ms}{\rho}
\newcommand{\sms}{\lambda}

%% Polynomials



\newcommand{\minDegree}{{\underline{\bdegree}}}
\newcommand{\maxDegree}{{\overline{\bdegree}}}





==> source_files/argyris_dimension.tex <==
\section{Dimension of $\splSpace^{\smooth,2\smooth}_{4\smooth+1}$}\label{sec:argyris_dimension}

==> source_files/ideal_homology.tex <==
\section{Homology of $\idealComplex$}\label{sec:ideal_homology}

==> source_files/pht_dimension.tex <==
\section{PHT-splines of mixed smoothness}\label{sec:pht}
In this section, let us present an application of Theorem \ref{thm:dimension} to a special space of splines called PHT-splines \cite{deng2008polynomial}.

\begin{definition}[PHT smoothness distribution]
	Let $\bsmoothp$ be a smoothness distribution such that for all segments $A  \subset \meshEH$ (resp., $\meshEV$), $\bsmoothp(\edge) \leq (\degreev-1)/2$ (resp., $(\degreeu-1)/2$) for all $\edge \in A$.
\end{definition}

\begin{theorem}[Mourrain \cite{mourrain2014dimension}]
	\begin{equation*}
		\dimwp{\splSpace^{\bsmoothp}} = \euler{\quotientComplex^{\bsmoothp}}\;.
	\end{equation*}
\end{theorem}


